IKEA Furniture Assembly Environment for Long-Horizon Complex Manipulation Tasks

The IKEA Furniture Assembly Environment is one of the first benchmarks for testing and accelerating the automation of complex manipulation tasks. The environment is designed to advance reinforcement learning from simple toy tasks to complex tasks requiring both long-term planning and sophisticated low-level control. Our environment supports over 80 different furniture models, Sawyer and Baxter robot simulation, and domain randomization. The IKEA Furniture Assembly Environment is a testbed for methods aiming to solve complex manipulation tasks. The environment is publicly available at https://clvrai.com/furniture

==> text/approach.tex <==
\section{Approach}

\begin{figure*}[t]
\centering
    \includegraphics[width=0.8\textwidth]{figure/model_temp.png}
    \caption{
        Our graph neural network augmented for hierarchical RL policies.
        To perform a complex task, our model iterates graph computation for relational reasoning.
        The attention module examines which node or edge to manipulate and the computed attention works as a high-level action. 
        Then, the policy module takes as input the attended edge embedding and computes the low-level action.
        \label{fig:model}
    }
\end{figure*}


In this paper, we address the problem of solving a complex task that requires relational reasoning and hierarchical planning.
We propose a hierarchical framework with a graph neural network that learns to extract spatial information and object interactions required to perform robotic manipulation skills.
In \secref{model}, we describe our framework in details. Next, in \secref{training}, we elaborate how our model is efficiently trained with curriculum learning.

\subsection{Preliminaries}
\label{sec:preliminary}
We formulate our problem as a Markov decision process defined by a tuple $\{\mathcal{S}, \mathcal{A}, \mathcal{T}, R, \rho, \gamma\}$ of states, actions, transition probability, reward, initial state distribution, and discount factor. 
An action distribution of an agent is represented as a policy $\pi_\theta(a_t|s_t)$, where $s_t \in \mathcal{S}$ is a state, $a_t \in \mathcal{A}$ is an action at time $t$, and $\theta$ are the parameters of the policy.
An initial state $s_0$ is randomly sampled from $\rho$, and then, an agent iteratively takes an action $a_t$ sampled from a policy $\pi_\theta(a_t|s_t)$ and receives a reward $r_t$ until the episode ends. 
The performance of the agent is evaluated based on a discounted return $R=\sum _{t=0}^{T-1}\gamma ^{t}r_{t}$, where $T$ is the episode horizon.


\subsection{Input Module}
\yw{CNN to encode a part image and an observation into a part representation.}
The input module encodes part images and observations into node embeddings for the graph neural network. The input module is composed of two CNN submodules. The first takes as input static part images and outputs node embeddings for each part. The second network takes in the scene observation and outputs a scene embedding. The node embeddings and the scene embeddings are then used as input for the graph neural network. 

\subsection{Relational Module with Graph Neural Network}
\label{sec:model}
The relational module aims to output a graph state representation where the nodes represent entities in the scene and edges represent relations between entities. We choose the graph neural network architecture to output this graph representation of the scene. 

\ed{Should this be moved to input module since it is about node embedding? or is this node embedding of GNN}
A node embedding in the graph neural network contains appearance and geometric information of each object, such as color, shape, fine-grained position, and rotation whereas an edge embedding represents relations between two or more objects and it is used for relational reasoning. 

\ed{Explain difference between node embeddings in GNN and part encoding of Input Module}
A graph neural network achieves better sample efficiency by sharing network for extracting a node embedding and edge embedding. However, even given a perfect graph representation of the state, it is still complicated for the policy module to decide low-level actions by taking all node and edge embeddings as input. 

To alleviate this problem, we attend over node and edge embeddings to focus on specific nodes and edges for the policy module. 
\ed{I don't understand this}
Then, the resulting attention map helps efficient optimization of the graph neural network which finds good representations for the policy using RL signal.


\subsection{Policy module}
We train a policy module that takes as input the attended graph output of the Relational module and outputs a low level action. The policy network predicts the low-level action based on the essential and relational information extracted by the graph neural network and the high-level action/relation computed by the attention network. 

We use Proximal Policy Optimization (PPO)~\cite{PPO}, a common choice for continuous control environments, to train the policy module.
The attention map from the attention module and context vector from the context module are fed to the policy module, and then the policy module outputs action probability and value prediction. 
The policy module consists of a recurrent neural network implemented using a Gated Recurrent Unit (GRU)~\cite{cho2014gru} to exploit temporal information and the output of the GRU is used as a representation for computing action and value.


\subsection{Curriculum Learning}
\label{sec:training}

We found that a curriculum learning boosts the training speed by a large margin. Hence, we follow the curriculum strategy of \citet{zaremba2015reinforcement}. 
Every episode, a task is mainly sampled from the task distribution, but specifically designed tasks for teaching subtasks are sampled with 0.3 probability. 
The training starts with tasks containing 2 objects which helps to learn basic rules of solving the problems. Moreover, we provide tasks for learning to pick, learning to align, and learning to attach two objects.

